On the nature of the black hole information problem

The aim of this work is to present the black hole information problem and discuss the assumptions and hypotheses necessary for its formulation. As the problem arises in the framework of semiclassical gravity, we first review the necessary notions to describe Lorentzian manifolds equipped with physical properties, as well as the physical concepts of the theory that describes the gravitational interaction as the curvature of spacetime, general relativity. From its classical perspective, we develop the formalism to study the dynamical aspects of black holes in spacetimes obeying suitable causality conditions. Equipped with conjectures that nature censors naked singularities and that black holes reach a stationary configuration after they form, the black hole uniqueness theorems allow us to review several relations for the geometrical quantities associated with them. Following considerations of the other fundamental interactions, which are described by quantum field theory, we review the arguments in the formalism of quantum field theory in curved spacetime that give rise to the effective particle creation effect, its approximately thermal character, and the concept of black hole evaporation. With a precise quantification of information in quantum mechanics and assuming that the condition for physically acceptable states is given by the Hadamard condition, we review the result that entanglement between causally complementary regions is an intrinsic feature of quantum field theory. As a consequence, we discuss how the formation and complete evaporation of black holes leads to information loss. Conscious that such a prediction follows if no deviations from the semiclassical picture occur at the Planck scale, we discuss alternatives to this nonunitary dynamical evolution and formulate the black hole information problem. Lastly, we analyze the assumptions and hypotheses that lead to the problem.

==> Post-text/Annex.tex <==
\begin{anexosenv}

% Imprime uma página indicando o início dos anexos
\partanexos

\end{anexosenv}


==> Pre-text/Abbreviations.tex <==
\begin{siglas}
    \item[ABNT] Associação Brasileira de Normas Técnicas
    \item[abnTeX] ABsurdas Normas para TeX
	\item[IBGE] Instituto Brasileiro de Geografia e Estatística
	\item[LaTeX] Lamport TeX
	\item[USP] Universidade de São Paulo
	\item[USPSC] Campus USP de São Carlos
\end{siglas}


==> Pre-text/Aprovacao.tex <==
%% USPSC-folhadeaprovacao.tex
% Alternativa para a Folha de Aprovação 
% Se esta for a sua opção, exclua inclusão feita acima do arquivo folhadeaprovacao.pdf
%
\begin{folhadeaprovacao}
  \begin{center}
       {\ABNTEXchapterfont\bfseries\large\imprimirautor}
	 \vspace*{2cm}
   
    \begin{center}
      \ABNTEXchapterfont\bfseries\Large\imprimirtitulo
    \end{center}
		\vspace*{2cm}
		\hspace{.45\textwidth}
    \begin{minipage}{.5\textwidth}
        \imprimirpreambulo
    \end{minipage}
		\vspace*{2cm}
    %\vspace*{\fill}
	\end{center}

  \begin{center}
	  {\ABNTEXchapterfont\bfseries\large\ {Data de defesa: 02 de outubro de 2015} \\}
		\vspace*{\fill}
	  {\ABNTEXchapterfont\bfseries\large\ {Comiss\~ao Julgadora:} \\}
		%Trabalho aprovado. \imprimirlocal, 2 de outubro de 2015:
		
		%\assinatura{\textbf{\imprimirorientador} \\ Orientador} 
		\assinatura{\textbf{\imprimirorientador} \\}
    % Se for ORIENTADOR, inclua % no início do comando abaixo e tire a % do próximo comando 
		\renewcommand{\orientadorname}{Orientadora}
		%\renewcommand{\orientadorname}{Orientador}

		\imprimirorientadorRotulo
		\par
		\assinatura{\textbf{Professor} \\ Convidado1}
	
		\assinatura{\textbf{Professor} \\ Convidado2}
		%\assinatura{\textbf{Professor} \\ Convidado3}
		%\assinatura{\textbf{Professor} \\ Convidado4}
		%\begin{center}
		\vspace*{\fill}
   	{\ABNTEXchapterfont\bfseries\large\imprimirlocal}
    \par
    {\ABNTEXchapterfont\bfseries\large\imprimirdata}
\end{center}
\end{folhadeaprovacao}
% ---

==> Pre-text/Capa.tex <==
%% USPSC-CapaICMC.tex
\AddToShipoutPicture{\BackgroundPic}
%-------------
\begin{minipage}[c]{144mm}
   \centering
   \begin{textblock*}{144mm}(61mm,65mm)
   \vspace*{1,2cm}
   \linespread{0.5}
   \ABNTEXchapterfont\bfseries\Large
   \textcolor{capa-azul}{\nohyphens{\imprimirtitulo}}
   \end{textblock*}
\end{minipage}
\vfill
\vspace*{5cm}
\begin{minipage}[t][65mm][t]{125mm}
   \begin{textblock*}{130mm}(81mm,123mm)
      \ABNTEXchapterfont\bfseries\Large
      \textcolor{capa-azul}{\nohyphens{\imprimirautor}} 
      \vfill
      \vspace{9pt}
      \ABNTEXsubsectionfontsize\small
      \renewcommand{\ABNTEXsubsectionfontsize}{\fontsize{10}{6}\normalfont}
      \ABNTEXsubsectionfontsize 
      \textcolor{capa-azul}{\nohyphens{\imprimirnotacapaicmc}}
      \renewcommand{\ABNTEXsubsectionfontsize}{\fontsize{12}{12}\normalfont}
   \end{textblock*}	
\end{minipage} 
% ---


==> Pre-text/Ficha.tex <==
%% USPSC-fichacatalografica.tex
% ---
% Inserir a ficha bibliografica
% ---
% Isto é um exemplo de Ficha Catalográfica, ou ``Dados internacionais de
% catalogação-na-publicação''. Você pode utilizar este modelo como referência. 
% Porém, provavelmente a biblioteca da sua universidade lhe fornecerá um PDF
% com a ficha catalográfica definitiva após a defesa do trabalho. Quando estiver
% com o documento, salve-o como PDF no diretório do seu projeto e substitua todo
% o conteúdo de implementação deste arquivo pelo comando abaixo:
%
\begin{fichacatalografica}
	\hspace{-1.4cm}
	\imprimirnotaautorizacao \\ \\
	%\sffamily
	\vspace*{\fill}					% Posição vertical
\begin{center}					% Minipage Centralizado
  \imprimirnotabib \\
  \begin{table}[htb]
	\scriptsize
	\centering	
	\begin{tabular}{|p{0.9cm} p{8.7cm}|}
		\hline
	      & \\
		  &	  \imprimirautorficha     \\
		
		 \imprimircutter & 
							\hspace{0.4cm}\imprimirtitulo~  / ~\imprimirautor~ ;  ~\imprimirorientadorcorpoficha. -- 	\imprimirlocal, \imprimirdata.   \\
		
		  &  % Para incluir nota referente à versão corrigida no corpo da ficha,
			  % incluir % no início da linha acima e tirar a % do início da linha abaixo
			  %	\hspace{0.4cm} \imprimirtitulo~  / ~\imprimirautor~ ; ~\imprimirorientadorcorpoficha~- ~\imprimirnotafolharosto. -- \imprimirlocal, \imprimirdata.  \\
		
			\hspace{0.4cm}\pageref{LastPage} p. : il. (algumas color.) ; 30 cm.\\ 
		  & \\
		  & 
		    \hspace{0.4cm}\imprimirnotaficha ~--~ 
						  \imprimirunidademin, 
						  \imprimiruniversidademin, 
		                  \imprimirdata. \\ 
		  & \\                 
		   % Para incluir nota referente à versão corrigida em notas,
		    % incluir uma % no início da linha acima e	
		    % tirar a % do início da linha abaixo
		    % & \hspace{0.4cm}\imprimirnotafolharosto \\ 
		  & \\ 
		  & \hspace{0.4cm}1. LaTeX. 2. abnTeX. 3. Classe USPSC. 4. Editoração de texto. 5. Normalização da documentação. 6. Tese. 7. Dissertação. 8. Documentos (elaboração). 9. Documentos eletrônicos. I. \imprimirorientadorficha. 
		   II. Título. \\
	
		     %Se houver co-orientador, inclua % antes da linha (antes de II. Título.) 
		     %          e tire a % antes do comando abaixo 
		     %III. Título. \\   
		  \hline
	\end{tabular}
  \end{table}
\end{center}
\end{fichacatalografica}
% ---



==> Pre-text/Symbols.tex <==
\begin{simbolos}
  \item[$ \mathcal{M} $] Minkowski spacetime
  \item[$T_{(\mu_{1}...\mu_{\ell})}$] Symmetric part of the tensor $T_{\mu_{1}...\mu_{\ell}}$ (see eq. \ref{symmetric})
  \item[$T_{[\mu_{1}...\mu_{\ell}]}$] Antisymmetric of the tensor $T_{\mu_{1}...\mu_{\ell}}$ (see eq. \ref{antisymmetric})
\end{simbolos}

==> USPSC-IndicesRemissivos.tex <==
%% USPSC-IndicexRemissivos.tex
% ---
% Inicia os Índices Remissivos
% ---
%---------------------------------------------------------------------
% INDICE REMISSIVO
%--------------------------------------------------------------------
\phantompart
\printindex
%---------------------------------------------------------------------


==> USPSC-pre-textual-IFSC.tex <==
%% USPSC-pre-textual-IFSC.tex
%% Camandos para definição do tipo de documento (tese ou dissertação), área de concentração, opção, preâmbulo, titulação 
%% referentes ao Programa de Pós-Graduação o IFSC
\instituicao{Instituto de F\'isica de S\~ao Carlos, Universidade de S\~ao Paulo}
\unidade{INSTITUTO DE F\'ISICA DE S\~AO CARLOS}
\unidademin{Instituto de F\'isica de S\~ao Carlos}
\universidademin{Universidade de S\~ao Paulo}

\notafolharosto{\center{Corrected version} \\ (Original version available on the Program Unit)}
% ---
% dados complementares para CAPA e FOLHA DE ROSTO
% ---
\universidade{UNIVERSIDADE DE S\~AO PAULO}
\titulo{On the nature of the black hole information problem}

\titleabstract{On the nature of the black hole information problem}
\tituloresumo{Sobre a natureza do problema da informação em buracos negros}
\autor{Thiago Torres Bergamaschi}
\autorficha{Bergamaschi, Thiago}
\autorabr{BERGAMASCHI, T. T.}

\cutter{S856m}
% Para gerar a ficha catalográfica sem o Código Cutter, basta 
% incluir uma % na linha acima e tirar a % da linha abaixo
%\cutter{ }

\local{S\~ao Carlos}
\data{2024}
% Quando for Orientador, basta incluir uma % antes do comando abaixo
\renewcommand{\orientadorname}{Orientadora:}
% Quando for Coorientadora, basta tirar a % utilizar o comando abaixo
%\newcommand{\coorientadorname}{Coorientador:}
\orientador{Prof. Dr. Esmerindo de Sousa Bernardes}
\orientadorcorpoficha{orientadora Elisa Gon\c{c}alves Rodrigues}
\orientadorficha{Rodrigues, Elisa Gon\c{c}alves, orient}
%Se houver co-orientador, inclua % antes das duas linhas (antes dos comandos \orientadorcorpoficha e \orientadorficha) 
%          e tire a % antes dos 3 comandos abaixo
%\coorientador{Prof. Dr. Jo\~ao Alves Serqueira}
%\orientadorcorpoficha{orientadora Elisa Gon\c{c}alves Rodrigues ;  co-orientador Jo\~ao Alves Serqueira}
%\orientadorficha{Rodrigues, Elisa Gon\c{c}alves, orient. II. Serqueira, Jo\~ao Alves, co-orient}

\notaautorizacao{I AUTORIZE THE REPRODUCTION AND DISSEMINATION OF TOTAL OR PARTIAL COPIES OF THIS DOCUMENT, BY CONVENCIONAL OR ELECTRONIC MEDIA FOR STUDY OR RESEARCH PURPOSE, SINCE IT IS REFERENCED.}
\notabib{Ficha catalogr\'afica revisada pelo Servi\c{c}o de Biblioteca e Informa\c{c}\~ao Prof. Bernhard Gross, com os dados fornecidos pelo(a) autor(a)}

\newcommand{\programa}[1]{

% DFAe ==========================================================================
\ifthenelse{\equal{#1}{DFAe}}{
	\renewcommand{\areaname}{Concentration area:}
	\renewcommand{\opcaoname}{Option:}
	\renewcommand{\orientadorname}{Advisor:}
	\tipotrabalho{Dissertaç\~ao (Mestrado em Ci\^encias)}
	\tipotrabalhoabs{Dissertation (Master's degree in Science)}
	\area{Theoretical and Experi-
mental Physics}
	%\opcao{Nome da Opção}
   	% O preambulo deve conter o tipo do trabalho, o objetivo, 
   	% o nome da instituição, a área de concentração e opção quando houver
   	\preambulo{Dissertation presented to the Graduate Program in Physics at the Instituto de F\'isica de S\~ao Carlos da Universidade de S\~ao Paulo, to obtain the degree of Master in Science.}
   	\notaficha{Dissertation (Master - Graduate Program in Applied Physics)}
    }{    
}}
				
				








==> USPSC-unidades.tex <==
%% USPSC-unidades.tex
% Camando para definição do programa de Pós-Graduação, Especialidade do Título e Instituição
\newcommand{\siglaunidade}[1]{


% EESC-TCC ==========================================================================
    \ifthenelse{\equal{#1}{EESC-TCC}}{
     			\include{USPSC-TCC-pre-textual-EESC}
% ---
    }{
% EESC ==========================================================================
	\ifthenelse{\equal{#1}{EESC}}{
	\include{USPSC-pre-textual-EESC}
	% ---
}{    
% IAU ===========================================================================
        \ifthenelse{\equal{#1}{IAU}}{
        \include{USPSC-pre-textual-IAU}    
        }{
% ICMC ===========================================================================
        \ifthenelse{\equal{#1}{ICMC}}{
        \include{USPSC-pre-textual-ICMC}    
        }{
% ICMC-TCC ===========================================================================
        \ifthenelse{\equal{#1}{ICMC-TCC}}{
        	\include{USPSC-TCC-pre-textual-ICMC}    
        }{
% IFSC ===========================================================================
        \ifthenelse{\equal{#1}{IFSC}}{
        \include{USPSC-pre-textual-IFSC}    
        }{
% IQSC ===========================================================================
        \ifthenelse{\equal{#1}{IQSC}}{
        \include{USPSC-pre-textual-IQSC}    
        }{
% IQSC-TCC ===========================================================================
	\ifthenelse{\equal{#1}{IQSC-TCC}}{
	\include{USPSC-TCC-pre-textual-IQSC}    
       }{
% USPSC ===========================================================================
\ifthenelse{\equal{#1}{USPSC}}{
	\include{USPSC-pre-textual-Tutorial}    
}{
% OUTROS-TCC ===========================================================================
\ifthenelse{\equal{#1}{OUTROS-TCC}}{
	\include{USPSC-TCC-pre-textual-OUTROS}    
}{
% Outros ========================================================================
                       % ------------------------------------------------------------------------
        \include{USPSC-pre-textual-OUTRO} 
								  }
                }
							}
						}
				}
			}}}}}}
         	

